Stable-TTS: Stable Speaker-Adaptive Text-to-Speech Synthesis via Prosody Prompting

Speaker-adaptive Text-to-Speech (TTS) synthesis has attracted considerable attention due to its broad range of applications, such as personalized voice assistant services. While several approaches have been proposed, they often exhibit high sensitivity to either the quantity or the quality of target speech samples. To address these limitations, we introduce Stable-TTS, a novel speaker-adaptive TTS framework that leverages a small subset of a high-quality pre-training dataset, referred to as prior samples. Specifically, Stable-TTS achieves prosody consistency by leveraging the high-quality prosody of prior samples, while effectively capturing the timbre of the target speaker. Additionally, it employs a prior-preservation loss during fine-tuning to maintain the synthesis ability for prior samples to prevent overfitting on target samples. Extensive experiments demonstrate the effectiveness of Stable-TTS even under limited amounts of and noisy target speech samples.

==> figures/mel_plot.tex <==
\begin{figure}[h]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=\linewidth]{figures/mel_plot_0312.pdf}
    \caption{\textbf{Visualization of Mel-spectrograms of Synthesized Speech.} Mel-spectrograms are depicted with enhanced resonant frequencies when the prior-preservation loss is applied.}
    \vspace{-0.25in}
    \label{fig:mel_plot}
\end{figure}
